Dynamic Clustering Algorithms via Small-Variance Analysis of Markov Chain Mixture Models

Bayesian nonparametrics are a class of probabilistic models in which the model size is inferred from data. A recently developed methodology in this field is small-variance asymptotic analysis, a mathematical technique for deriving learning algorithms that capture much of the flexibility of Bayesian nonparametric inference algorithms, but are simpler to implement and less computationally expensive. Past work on small-variance analysis of Bayesian nonparametric inference algorithms has exclusively considered batch models trained on a single, static dataset, which are incapable of capturing time evolution in the latent structure of the data. This work presents a small-variance analysis of the maximum a posteriori filtering problem for a temporally varying mixture model with a Markov dependence structure, which captures temporally evolving clusters within a dataset. Two clustering algorithms result from the analysis: D-Means, an iterative clustering algorithm for linearly separable, spherical clusters; and SD-Means, a spectral clustering algorithm derived from a kernelized, relaxed version of the clustering problem. Empirical results from experiments demonstrate the advantages of using D-Means and SD-Means over contemporary clustering algorithms, in terms of both computational cost and clustering accuracy.

==> background-arxiv.tex <==
\section{Temporally Varying Cluster Model} %Background: The Markov Dependent Dirichlet Process}
The Dirichlet process (DP) is a prior over discrete probability
measures~\citep{Sethuraman94_SS, Ferguson73_ANSTATS}. In general,
if $D$ is DP distributed, then realizations are probability measures
$D = \sum_k \pi_k \delta_{\theta_k}$ consisting of a countable number 
of discrete atoms $\delta_{\theta_k}$, each with measure $1$ and location
$\theta_k$ in some space, and weights $\pi_k$, with $\sum_k \pi_k =
1$~\citep{Sethuraman94_SS}. We denote $D \sim \text{DP}(\alpha \mu)$, where
$\alpha$ is the \emph{concentration parameter} that determines how
the weights $\pi_k$ are distributed amongst the atoms, while
$\mu$ is the \emph{base measure} from which atom locations $\theta_k$ are
sampled independently. When used as a prior over mixture models,
the locations $\theta_k$ can be thought of as the parameters of the clusters,
while the weights $\pi_k$ are the weights in the categorical distribution of
labels. The
reader is directed to~\citep{Teh10_EML} for a more thorough coverage of Dirichlet
processes.

The dependent Dirichlet process (DDP), an extension to the DP, is a prior over 
covariate-dependent discrete probability measures~\citep{MacEachern99_ASA}. One
particularly useful construction of the DDP, the Markov dependent Dirichlet
process (Markov DDP), forms a Markov chain of DPs
($D_1, D_2, \dots$), where
the transitions are governed by a set of three stochastic operations~\citep{Lin10_NIPS}: 
atoms $\delta_{\theta_k}$ may be added, removed, and may move during 
each step of the Markov chain. Thus, their locations become parameterized by time, denoted
by $\theta_{kt}$. If the DDP is used as a prior over a mixture model, these three operations allow
new mixture components to arise over time, and old mixture components to exhibit dynamics
and perhaps disappear over time. The reader is directed to~\citep{Lin10_NIPS},
for a more thorough coverage of this construction of the DDP. 

%In slightly more detail, if $D_{t}$ is the DP at time
%step $t$, then the following procedure defines the generative model of $D_t$ conditioned
%on $D_{t-1} \sim \mathrm{DP}(\mu_{t-1})$:
%\begin{enumerate}
%  \item{\textbf{Subsampling}:
%    Define a function $q : \Omega \rightarrow [0,1]$. Then for each point
%    $(\theta, \pi) \in D_{t-1}$, sample a Bernoulli distribution $b_\theta \sim
%    \mathrm{Be}(q(\theta))$. Set $D'_t$ to be the collection of points $(\theta, \pi)$ such
%    that $b_\theta = 1$, and renormalize the weights. Then $D'_t \sim
%    \mathrm{DP}(q\mu_{t-1})$, where $(q\mu)(A) = \int_A q(\theta)\mu(d\theta)$.
%  }
%  \item{\textbf{Transition}: Define a distribution $T : \Omega \times \Omega
%    \rightarrow \mathbb{R}_+$. For each point $(\theta, \pi)\in D'_t$, 
%    sample $\theta' \sim T(\theta' | \theta)$, and set $D''_t$ to be 
%    the collection of points $(\theta', \pi)$. Then $D''_t \sim
%    \mathrm{DP}(Tq\mu_{t-1})$, where $(T\mu)(A) = \int_A\int_\Omega T(\theta' |
%    \theta) \mu(d\theta)$.
%  }
%  \item{\textbf{Superposition}: Sample $F \sim \mathrm{DP}(\nu)$, and
%    sample $(c_D, c_F) \sim \mathrm{Dir}(Tq\mu_{t-1}(\Omega), \nu(\Omega))$. 
%    Then set $D_t$ to be the union of $(\theta, c_D\pi)$ for all $(\theta, \pi)
%    \in D''_t$ and $(\theta, c_F\pi)$ for all $(\theta, \pi)\in F$. Thus,
%    $D_t$ is a random convex combination of $D''_t$ and $F$, where
%    $D_t \sim \mathrm{DP}(Tq\mu_{t-1} + \nu)$.
%  }
%\end{enumerate}

An important result of using such a construction is the development of
an explicit posterior for $D_t$ given observations
$\{\theta'_{it}\}_{i=1}^{N_t}$ sampled from $D_t$ of the points $\theta_{kt}$ at
timestep $t$. For each point $k$
that was observed in $D_{\tau}$ for some $\tau : 1\leq \tau \leq t$, define:
$n_{kt}\in\mathbb{N}$ as the number of observations of point $k$ in timestep
$t$; $c_{kt}\in\mathbb{N}$ as the number of past observations of point $k$ 
prior to timestep $t$,
i.e.~$c_{kt} = \sum_{\tau = 1}^{t-1} n_{k \tau}$; $q_{kt}\in(0, 1)$ as
the prior probability that atom $k$ is not destroyed during timestep $t$; 
and $\dtk$ as the 
number of time steps that have elapsed since point $k$ was last observed. 
Further, let $\nu_t$ be 
the measure for unobserved points at time step $t$, and $\alpha_t$ be the
concentration parameter at time $t$.
Then,
\begin{align}
  D_t | D_{t-1}, \{\theta'_{it}\}_{i=1}^{N_t}  &\sim \text{DP}\left(\alpha_t\nu_t +
  \sum_{k : n_{kt} = 0}q_{k t} c_{k t} T(\cdotp|\theta_{k(t-\dtk)}) + \sum_{k : n_{kt} >
0} (c_{k t} + n_{k t})\delta_{\theta_{kt}}\right),\label{eq:ddpposterior}
\end{align}
where $c_{kt} = 0$ for any point $k$ that was first observed during
timestep $t$. The first term in the posterior accounts for clusters
that have not been observed yet; the second term accounts for clusters
that were previously seen but not instantiated in the present time step;
and the last accounts for clusters that are currently instantiated. 

%This posterior leads directly
%to the development of a Gibbs sampling algorithm for the DDP,
%whose small-variance asymptotics are discussed further below.


==> dmeansmonoproof-arxiv.tex <==
\section{Proof of Monotonicity in the D-Means Clustering Cost}\label{app:dmeansmonoproof}
\begin{proofof}{Theorem \ref{thm:dmeansmono}}
This proof proceeds by showing that each step of Dynamic Means 
(parameter assignment and label assignment) individually do not 
increase $J_t$. Thus, when these steps are iterated, $J_t$ is 
monotonically decreasing.

The first step considered is the parameter update. During
this update, the portion of $J_t$ attributed to $\lambda$ and
$Q$ does not change, as the cluster labels are held constant. Therefore,
the only portion of $J_t$ that needs to be considered is the weighted
sum square cost. Taking the derivative of this with respect to
$\theta_{kt}$, and setting it equal to 0 yields 
\begin{align}
  \begin{aligned}
  0 &= \gamma_{kt}(\theta_{kt} - \theta_{k(t-\dtk)}) + \sum_{z_{it}=k}
  (\theta_{kt} - y_{it})\\
  (\gamma_{kt} + n_{kt}) \theta_{kt} &= \gamma_{kt}\theta_{k(t-\dtk)} +
  \sum_{z_{it} = k} y_{it}\\
  \theta_{kt} &= \frac{\gamma_{kt}\theta_{k(t-\dtk)} +
  n_{kt}m_{kt}}{\gamma_{kt} + n_{kt}},
  \end{aligned}
\end{align}
and since this portion of the cost function is convex in $\theta_{kt}$,
this is the minimizing $\theta_{kt}$ for cluster $k$, and thus this
portion of the cost function is reduced. Note that if $k$ is a newly
created cluster in timestep $t$, $\gamma_{kt} = 0$ and thus $\theta_{kt}$
is set to the current sample mean, $m_{kt}$.


The second step considered is the label update. Here, there are a number of
cases: 1) the update moves an observation from a currently active cluster to
another currently active cluster; 2) the update creates a new cluster; 3) the
update revives an old cluster; and 4) the observation was the last in its 
group, and the cluster is destroyed. Each case will be considered separately.
Note that the amount that an observation $y$ in cluster $k$ 
contributes to the cost function prior to reassignment is $\|y - \theta_{kt}\|^2$.
\begin{enumerate}
  \item {Suppose the observation $y$ in cluster $k$ becomes
assigned to a currently active cluster $j$. 
Since the cluster was already active, the observation now
contributes $\|y-\theta_{jt}\|^2$ to the cost, and $\|y -
\theta_{jt}\|^2 \le \|y - \theta_{kt}\|^2$ because the label
assignment step chose the minimum of these two. Thus, the cost does not
increase.}
  \item{Suppose the observation $y$ in cluster $k$ is assigned to a brand new
      cluster $K$ with cost $\lambda$ (the
      new $\|y-\theta_{Kt}\|^2$ cost is $0$, since $\theta_{Kt}$ is set to
      $\theta_{Kt}=y$ when a new cluster is created). Then 
      we know that $\lambda +\|y-\theta_{Kt}\|^2 = \lambda \leq \|y - \theta_{kt}\|^2$ due to the 
label assignment step choosing the minimum of these two, and thus the cost does
not increase.}
\item{Suppose the observation $y$ in cluster $k$ revives an old cluster $j$.
    Then
\begin{align}
  \frac{||y - \theta_{j(t-\dtk)}||_2^2}{ \dtj \tau + 1} + Q\dtj
  \leq ||y - \theta_{kt} ||_2^2,
\end{align}
and further, using the parameter update (\ref{eq:paramupdate}), 
\begin{align}
  \theta_{jt} = \frac{\theta_{j(t-\dtk)}\gamma_{jt} + y} {\gamma_{jt} + 1 }.
\end{align}
Rearranging the above yields two relations:
\begin{align}
  \begin{aligned}
  ||\theta_{jt} - y ||_2^2 &= \frac{\gamma_{jt}^2}{ \left(1+\gamma_{jt}\right)^2} || \theta_{j(t-\dtj)}-y ||_2^2\\
  ||\theta_{jt} - y ||_2^2 &= \gamma_{jt}^2||\theta_{jt} -
  \theta_{j(t-\dtj)}||_2^2,
  \end{aligned}
\end{align}
where $\gamma_{jt} = \left( (w_{j(t-\dtj)})^{-1} +  {\Delta
t}_{j}\tau\right)^{-1}$. Placing these terms in a weighted least-squares-like
configuration yields
\begin{align}
  \begin{aligned}
||\theta_{jt} - y ||_2^2 + \gamma_{jt}||\theta_{jt} - \theta_{j(t-\dtj)}||_2^2 &= (1+\gamma_{jt}^{-1})||\theta_{jt} - y ||_2^2\\
  &= \frac{(1+\gamma_{jt}^{-1})\gamma_{jt}^2}{(1+\gamma_{jt})^2}|| \theta_{j(t-\dtj)}-y ||_2^2\\
  &= \frac{1}{1+\gamma_{jt}^{-1}}|| \theta_{j(t-\dtj)}-y ||_2^2,
  \end{aligned}
\end{align}
and subbing in for the $\gamma_{jt}$ term, 
\begin{align}
  \begin{aligned}
||\theta_{jt} - y ||_2^2 + \gamma_{jt}||\theta_{jt} - \theta_{j(t-\dtj)}||_2^2 &= \frac{1}{1 +  (w_{j(t-\dtj)})^{-1} +  \dtj\tau} || \theta_{j(t-\dtj)}-y ||_2^2\\
    &\leq \frac{|| \theta_{j(t-\dtj)}-y ||_2^2}{1 +   \dtj\tau}. 
  \end{aligned}
\end{align}
Therefore, if the DDP k-means algorithm instantiates an old cluster,
\begin{align}
  \begin{aligned}
||\theta_{jt} - y ||_2^2 + \gamma_{jt}||\theta_{jt} - \theta_{j(t-\dtj)}||_2^2 +
Q \dtj &\leq \frac{||y - \theta_{j(t-\dtk)}||_2^2}{ \dtj \tau + 1} + Q\dtj\\
  &\leq ||y - \theta_{kt} ||_2^2,
  \end{aligned}
\end{align}
and the new contribution to the cost is less than the old contribution.}
\item{Suppose the observation $y$ in cluster $k$ was the last observation in its cluster prior 
to reassignment, and $y$ became assigned to a different cluster. 
If $y$ was previously part of a newly created cluster in this 
time step, the cost decreases by $\lambda$ after $y$ is reassigned; 
likewise, if $y$ was previously part of a revived cluster, the 
cost decreases by 
$Q\dtk + \gamma_{kt}\|\theta_{kt}-\theta_{k(t-\dtj)}\|^2$. 
Thus, the removal of a cluster that becomes empty after reassignment 
does not increase the cost.}
\end{enumerate}

\end{proofof}



==> expt-robot-arxiv.tex <==
\subsection{Robotic Interactions} 
The final experiment was designed to illustrate the advantages of using SD-Means
over D-Means or DDP mixture model Gibbs sampling when the relationships between datapoints are better expressed
as pair-wise similarities, rather than distances to cluster centers.
In particular, the experiment involved clustering noisy sets of obsrvations $\{(x_t,
  \dot{x}_t)\}_{t=1}^{T}$ from
an unknown number $K$ of latent dynamical systems $\dot{x} = f_k(x)$, $k=1, \dots, K$
in order to discover the latent functions $f_k(\cdot)$ modelled
as Gaussian processes (GPs). 

Clustering GPs is problematic for many inference algorithms 
for a number of reasons. Algorithms that update cluster parameters (such as
DP-GP Gibbs sampling~\citep{Joseph11_AR}) require
the inversion of a kernel matrix, which is computationally intractable for large datasets.
Many other algorithms, such as D-Means, require discretization of the GP
in order to compute distances, which incurs an exponential growth in
computational complexity with the input dimension of the GPs, 
and a linear growth with the output dimension. In practice, 
the increase in dimensionality also leads to increased
susceptibility to convergence to poor local optima. SD-Means has neither of these limitations, as similarity computations
do not require discretization, and cluster parameters are not instantiated
while clustering each batch of data.

The particular hardware setup for this experiment is as follows.
Two mobile robots $r\in\{1, 2\}$ (shown in Figure \ref{fig:robits})
drove on a 2-dimensional plane with
positional state $x_r, y_r$ and rotational state $\theta_r$ governed by the
speed and turn rate inputs $v_r, \phi_r$ through unicycle dynamics
\begin{align}
  \dot x_r &= v_r \cos (\theta_r) && \dot y_r = v_r \sin (\theta_r) &&
  \dot \theta_r = \phi_r
\end{align}
Robot 1 was controlled via joystick, and robot 2 was controlled 
autonomously with inputs $(v_2, \phi_2)$ that were a function $(v_2, \phi_2) =
f_k(\Delta x = x_2- x_1, \Delta y = y_2 - y_1, \theta_1, \theta_2)$ of the state of both robots. 
There were $K=14$ different latent dynamics that governed the interaction of
robot 2 with robot 1. The dataset was collected by a motion capture system,
and consisted of XX observed trajectories
(each trajectory was from a single interaction type $k$). 

The dataset was clustered in batches of XX observation sets by SD-Means, D-Means,
and DDP-GP Gibbs sampling. For SD-Means, the similarity function
for a pair of sets of observations $\{x_{1t}, \dot{x}_{1t}\}_{t=1}^{T_1}$, $\{x_{2t},
\dot{x}_{2t}\}_{t=1}^{T_2}$ was the probability that
both sets of observations were generated by a single GP, thresholded below by
$0.75$. For D-Means, the GP for each observation set was discretized to 10
points in each dimension, producing a feature vector of 
length 20,000 ($2\times 10^4$ for 4 input dimensions, 2 output dimensions). 
For DDP-GP, the Gibbs sampling algorithm for DP-GP~\citep{Joseph11_AR} was adapted to
the DDP prior.



The similarity graph for the dataset is shown in Figure~\ref{fig:motiongraphfull}, with node color denoting the true interaction
dynamics $f_k$ for each interaction segment. Each batch of data (e.g.~shown in Figure~\ref{fig:motiongraphstep}) was constructed from 70 segment GPs. While the
cluster structure of the dataset is relatively clear in Figure~\ref{fig:motiongraphfull}, much of that information is lost in Figure~\ref{fig:motiongraphstep}. Behaviors are missing entirely, and those that are present exhibit
incorrect connections. Many nodes are singletons, which confounds the clustering
process further. This creates a significant challenge for 
clustering algorithms that do not process the full dataset at once.

This difficulty manifests itself in the results of the experiment, shown in Table
\ref{tab:motionresults}. As expected, the batch algorithm outperforms all the
others, at the cost of intractability with
increasing dataset size, and an imposed artificial upper bound on
the number of clusters from using an approximate eigendecomposition. 
Compared to the other incremental algorithms, however,
SD-Means provided a significant improvement in clustering accuracy.
%BAT had the highest accuracy because it had access to all the information at
%once, and the interaction behaviors were not changing over time. 
\begin{figure}[t]
  \captionsetup{font=scriptsize}
  \begin{subfigure}[b]{0.38\columnwidth}
      \centering
      \includegraphics[width=0.9\columnwidth]{figures/robot/robits.png}
      \caption{}\label{fig:robits}
    \end{subfigure}
    \begin{subtable}[b]{0.6\columnwidth}
    \centering
    {\small \begin{tabular}{l|c|l}
      \textbf{Alg} & \textbf{\% Acc} & \textbf{Time (s)}\\
      \hline
      \rule{0pt}{9pt}\textbf{SD-Means}  & \textbf{39.0} & \textbf{2.70}\\
      D-Means   & 20.4          & 0.09\\
      PCM  & 16.1          & 0.17\\
      PCQ  & 12.7          & 0.71 \\
      IS   & 5.9           & 3.92\\
      %GS  & o             & s\\
      \hline
      \rule{0pt}{9pt}BAT  & 88.7          & 6.86
    \end{tabular}}
  \caption{}\label{tab:motionresults}
    \end{subtable}
    \begin{subfigure}[b]{0.49\columnwidth}
      \centering
      \includegraphics[width=2.5cm]{figures/robot/motiongraphfull.png}
      \caption{}\label{fig:motiongraphfull}
    \end{subfigure}
   \begin{subfigure}[b]{0.49\columnwidth}
     \centering
     \includegraphics[width=2.5cm]{figures/robot/motiongraphstep.png}
      \caption{}\label{fig:motiongraphstep}
    \end{subfigure}
        \caption{\ref{fig:robits}: The two robots. \ref{fig:motiongraphfull} -
    \ref{fig:motiongraphstep}: Similarity graphs for  the full robotic interaction data set with
      1400 nodes and for a single batch of 70 nodes.
      \ref{tab:motionresults}: The table of accuracy results and CPU
      time.}\label{fig:interactiongraph}
\end{figure}



==> expt-traj-arxiv.tex <==
\subsection{MIT Parking Lot Trajectories}


==> kerneldynamicmeans-arxiv.tex <==
\section{Kernel Dynamic Means (KD-Means)}\label{sec:kdmeans}
\subsection{Algorithm Description}
Similar to D-Means, Kernelized Dynamic Means\footnote{Code available online:
\url{http://github.com/trevorcampbell/dynamic-means}} (KD-Means) is an iterative algorithm 
that approximately solves the clustering problem (\ref{eq:krnmin}) via coordinate descent.
The algorithmic steps are the same as those in Algorithm \ref{alg:dynmeans}, except for 
two details: there is no separate parameter update step,
as it is wrapped into the label update (\ref{eq:krnlabelupdate}),
and $\phi_{kt}$ is updated to $\phi_{k(t+1)}$ approximately using sparse
regressor selection (\ref{eq:krnphiupdate})
rather than linear combination (\ref{eq:wupdate}). 

\paragraph{Label Update}
The minimum cost label assignment for datapoint $y_{it}$ is found by fixing all
other labels and computing the cost for assignment to each instantiated,
uninstantiated, and new cluster. First, $y_{it}$ is deassigned from its current
cluster $k$, so that $\indices_{kt} \gets \indices_{kt}\setminus \{i\}$, and
$n_{kt} \gets n_{kt}-1$. Then the optimal label $z_{it}$ is computed using
\begin{align}
  \begin{aligned}
  z_{it} =& \argmin_{k}
          \left\{\begin{array}{l l}
            J_{ik} 
            \quad &k\in\clusa_t\\
          Q\dtk +
          \frac{\gamma_{kt}}{\gamma_{kt}+1}\left(\krnmat{\Phi}{\Phi}_{kk}-2\krnmat{Y}{\Phi}_{ik}+\krnmat{Y}{Y}_{ii}\right) \quad & k \notin \clusa_t\\
            \lambda \quad & k = K_t+1
        \end{array}\right.\\  
        \text{where } J_{ik} =& \frac{(\gamma_{kt}+n_{kt})\krnmat{Y}{Y}_{ii}}{\gamma_{kt}+n_{kt}+1}
              -\frac{2\left(\gamma_{kt}\krnmat{Y}{\Phi}_{ik}
              +\sum_{j\in\indices_{kt}}\krnmat{Y}{Y}_{ij}\right)}{\gamma_{kt}+n_{kt}+1}\\
              +&\frac{\gamma_{kt}^2\krnmat{\Phi}{\Phi}_{kk}}{(\gamma_{kt}+n_{kt})(\gamma_{kt}+n_{kt}+1)}
              +\sum\limits_{j\in\indices_{kt}}\frac{2\gamma_{kt}\krnmat{Y}{\Phi}_{jk}+\sum_{l\in\indices_{kt}}\krnmat{Y}{Y}_{jl}}{(\gamma_{kt}+n_{kt})(\gamma_{kt}+n_{kt}+1)}
            \, .
\label{eq:krnlabelupdate}
  \end{aligned}
\end{align}

\paragraph{Old Center Update}
After the clustering is complete,
the regressor selection optimization (\ref{eq:krnphiupdate})
can be solved exactly with branch-and-bound~\citep{Bertsimas09_COA},
or approximately with greedy selection or 
an $l_1$-relaxation and coordinate descent~\citep{Bradley11_ICML}.

%This optimization is intractable to solve exactly due to the cardinality
%constraint. Therefore the solution is approximated with a simple greedy
%incremental subset selection procedure, shown in Algorithm
%\ref{alg:greedyselection}.
%
%\begin{algorithm}[t!]
%      \captionsetup{font=small}
%      \caption{Greedy Sparse Regressor Selection}
%      \small
%      \begin{algorithmic}
%        \Require $W \in \mathbb{R}^{(m+n_{kt})\time(m+n_{kt})},
%        \bar{a}\in\mathbb{R}^{m+n_{kt}}$ 
%        \State $c_0\gets \bar{a}^TW\bar{a}$, $c\gets c_0$
%        \State $w \gets W\bar{a}$
%        \State $\mathcal{J} \gets \{1, \dots, m+n_{kt}\}$
%    \For{$i = 1 \to m$}
%    \State $j^\star \gets \argmax_{j\in \mathcal{J}} w_j^2/W_{jj}$
%    \State $\mathcal{J} \gets \mathcal{J}\setminus\{j^\star\}$
%    \State $c\gets c-w_{j^\star}^2/W_{j^\star j^\star}$
%    \State $w \gets w - w_{j^\star}W_{:, j^\star}/W_{j^\star j^\star}$
%    \State $W \gets W-W_{:, j^\star}W_{j^\star, :}$
%  \EndFor 
%    \State $\mathcal{I} \gets \{1, \dots, m+n_{kt}\}\setminus \mathcal{J}$
%    \State \Return $\mathcal{I}$,
%    $W_{\mathcal{I}\mathcal{I}}^{-1}W_{\mathcal{I}\mathcal{J}}\bar{a}$, $\sqrt{c/c_0}$
%  \end{algorithmic}
%\end{algorithm}

\subsection{Analysis}
As with D-Means, KD-Means is guaranteed to converge to a local clustering 
cost minimum via typical monotonicity arguments. Furthermore, 
the successive application of the approximation (\ref{eq:krnphiupdate})
is stable in the sense that relative error between the true old center
and its approximation does not grow without bound over time, as
shown by Theorem \ref{thm:phierrorbound}.
\begin{theorem}\label{thm:phierrorbound}
  Let $\phi^\star_{kt}$ be the true old
  center $k$ at time $t$ given by (\ref{eq:phiexpansion}),
  and $\phi_{kt}$ be the approximation given by 
  (\ref{eq:krnphiupdate}). If
  after every time step, (\ref{eq:krnphiupdate})
  is solved with objective value less than $\epsilon^2$,
  i.e.~$(\bar{a}-a^\star)^TW(\bar{a}-a^\star) <\epsilon^2$, 
  then $\|\phi_{kt}-\phi^\star_{kt}\|_2 < \epsilon
  \left(1+\frac{1}{\tau}\right)\, \, \forall t \in \mathbb{N}$.
\end{theorem}
\begin{proof}
  See Appendix \ref{app:phiapproxproof}.
\end{proof}

\subsection{Practical Aspects and Implementation}
\subsubsection{Initialization}
As with all kernelized methods, the initialization of KD-Means 
has a strong influence on its performance.
Using a random ordering for introducing labels (as in D-Means)
can cause a large number of spurious clusters to be created.
Instead, during the first labelling pass over the data,
the next datapoint selected should be that which is closest to 
an already instantiated cluster. In this manner, new clusters 
are only introduced when they are absolutely 
required.


==> kernelization-arxiv.tex <==
\section{Kernelization of the Small-Variance MAP Filtering Problem}\label{sec:kernelization}
D-Means tends to perform best when the clusters are roughly 
spherical and linearly separable. While it is possible to redefine the cost 
equation (\ref{eq:DMeansObj}) in terms of more general distance metrics or
divergences~\citep{Banerjee05_JMLR}, clusters still must be spherical and
linearly separable using whichever distance metric or divergence is
chosen. When this assumption is violated, D-Means tends to create too many or
too few clusters to properly explain the data.

One way to extend the applicability of D-Means is by through
\emph{kernelization}~\citep{Dhillon07_TPAMI,Hofmann08_ANSTATS} of
the small-variance MAP filtering problem (\ref{eq:DMeansObj}).
Rather than clustering data vectors themselves at each time step,
a nonlinear embedding map is first applied to the vectors, and the embedded data 
is clustered instead. Crucially, the embedding map need not be known explicitly;
it is specified implicitly through a kernel function. Given an appropriate
kernel function, nonlinearly separable and nonspherical clusters in the original
data vector space become spherical and linearly separable in the embedding
space, thereby allowing the use of D-Means in this space. 
Thus, the goal of this section is to extend the applicability of D-Means beyond spherical, linearly
separable clusters via kernelization of the small-variance MAP filtering 
problem for the Markov DDP Gaussian mixture.

\subsection{Kernelization of the Cost}
Instead of clustering the data vectors directly, suppose 
we first map the vectors via the nonlinear embedding $\omega : \mathbb{R}^d
\to \mathbb{R}^n$. Then the least squares minimizer for the 
cluster centers in the new space is
\begin{align}
  \theta_{kt} &= \frac{\gamma_{kt}\phi_{kt} +
  \sum_{i\in\indices_{kt}}\omega(y_{it})}{\gamma_{kt}+n_{kt}} \in \mathbb{R}^n.\label{eq:nonlineartheta}
\end{align}
Substituting (\ref{eq:nonlineartheta}) and replacing $y_{it}$ with its nonlinear
embedding $\omega(y_{it})$ in (\ref{eq:DMeansObj}) yields the following 
clustering problem:
\begin{align}
\begin{aligned}
  \min_{\mathbf{z}_t} \sum_{i=1}^{N_t} \krnmat{Y}{Y}_{ii} + \sum_{k\in\clusa_t}
  \!\lambda\ind{\dtk}+Q\dtk+
    \frac{\gamma_{kt}n_{kt}\krnmat{\Phi}{\Phi}_{kk}}{\gamma_{kt}+n_{kt}} 
    -\!\sum_{i\in\indices_{kt}}\!\frac{2\gamma_{kt}\krnmat{Y}{\Phi}_{ik}+\sum_{j\in\indices_{kt}}\krnmat{Y}{Y}_{ij}}{\gamma_{kt}+n_{kt}}
  \end{aligned}\label{eq:krnmin}
\end{align}
where $\krnmat{Y}{Y}_{ij} = \omega(y_{it})^T\omega(y_{jt})$,
$\krnmat{Y}{\Phi}_{ik} = \omega(y_{it})^T\phi_{kt}$, and
$\krnmat{\Phi}{\Phi}_{kk} = \phi_{kt}^T\phi_{kt}$. Since $\phi_{kt}$ is not
known (as it lies in the embedding space), computing $\krnmat{Y}{\Phi}$
and $\krnmat{\Phi}{\Phi}$ requires that $\phi_{kt}$ is expressed
in terms of past data assigned to cluster $k$, 
\begin{align}
  \phi_{kt} &=
  \sum_{\tau\in\mathcal{T}_k}\left(\frac{1}{\gamma_{k\tau}}\prod_{r\in\mathcal{T}_k
  :
r \geq \tau}\frac{\gamma_{kr}}{\gamma_{kr}+n_{kr}}\right)
  \sum_{i\in\indices_{k\tau}}\omega(y_{i\tau}),
  \label{eq:phiexpansion}
\end{align}
where $\mathcal{T}_k$ is the set of all past timesteps where cluster $k$ was
active. Note
that the entire cost may now be specified in terms of dot products of data vectors in the embedding
space. Therefore, only the \emph{kernel function} $\krn{\cdot}{\cdot}
\!:\!\mathbb{R}^d\times \mathbb{R}^d
\to \mathbb{R}$ needs to be known, with the nonlinear embedding $\omega$ left
implicit.

\subsection{Recursive Approximation of Old Cluster Centers}
An issue with the above procedure is that computing $\krnmat{Y}{\Phi}$ and
$\krnmat{\Phi}{\Phi}$ via (\ref{eq:phiexpansion}) requires storing and computing
the kernel function with all past data. Over time, as the amount of 
observed data increases, this becomes intractable. Therefore, we instead
recursively approximate $\phi_{kt}$ with a linear combination of
a sparse subset of past data assigned to cluster $k$. Suppose
there is an approximation budget of $m$ past data vectors, and $\phi_{kt}$ 
is approximated as
\begin{align}
  \phi_{kt} &\simeq \sum_{j=1}^m a_j \omega(u_j),
\end{align}
where $a_j \in \mathbb{R}$, and $u_j \in \mathbb{R}^d$ (subscripts
$k$ and $t$ are suppressed for brevity). Then after
clustering the data $\{\omega(y_{it})\}_{i=1}^{N_t}$ at time $t$,
if $k\in\clusa_t$ the old center $\phi_{k(t+1)}$ is updated via
\begin{align}
  \phi_{k(t+1)} \simeq
  \frac{\gamma_{kt}\sum_{j=1}^m a_j
  \omega(u_j)+\sum_{i\in\indices_{kt}}\omega(y_{it})}{\gamma_{kt}+n_{kt}} =
  \sum_{j=1}^{m+n_{kt}} \bar{a}_j\omega(v_j)
  \label{eq:phiinitapprox}
\end{align}
where $\{u_j\}_{j=1}^m\bigcup\{y_{it}\}_{i\in\indices_{kt}}$ have been renamed
$\{v_j\}_{j=1}^{m+n_{kt}}$, $\bar{a}_j=
\frac{\gamma_{kt}}{\gamma_{kt}+n_{kt}} a_j \, \forall 1\leq j \leq m$, 
and $\bar{a}_{j} = \frac{1}{\gamma_{kt}+n_{kt}} \, \forall m+1\leq j \leq m+n_{kt}$.
As (\ref{eq:phiinitapprox}) requires storing $m+n_{kt}$ vectors, $\phi_{k(t+1)}$ must
be reapproximated with a subset containing $m$ vectors. This is accomplished
by solving a sparse regressor selection problem, 
\begin{align}
  \begin{aligned}
a^\star &\gets 
\argmin_{x\in\mathbb{R}^{m+n_{kt}}, \, \mathrm{card}(x) \leq m} 
  \left(\bar{a}-x\right)^TW\left(\bar{a}-x\right)\\
  \phi_{k(t+1)} &\gets\hspace{-.3cm} \sum_{j : |a^\star_j|> 0}\hspace{-.3cm}
a^\star_j\omega(v_j) \, \, .
  \end{aligned}
\label{eq:krnphiupdate}
\end{align}
where $W \in \mathbb{R}^{(m+n_{kt})\times (m+n_{kt})}$, $W_{ij} = \omega(v_i)^T\omega(v_j) = \krn{v_i}{v_j}$.



==> mapcostproof-arxiv.tex <==
\section{Proof of the Equivalence Between the D-Means Minimization and
  Small-Variance DDP-GMM MAP
Estimation}\label{app:mapcostproof}
\begin{proofof}{Theorem \ref{thm:mapcost}}
  The joint probability of the data, assignments, and clusters means can be
  broken into 3 components via Bayes' rule -- the data likelihood, and the priors
  on the parameters and assignments as follows:
  \begin{align}
    p\left(\{y_{it}\}_{i=1}^{N_t}, \{z_{it}\}_{i=1}^{N_t},
    \{\theta_{kt}\}_{k=1}^{K_t}\right) &=
     p\left(\{z_{it}\}_{i=1}^{N_t}\right)
    \prod_{i=1}^{N_t}p\left(y_{it}|\theta_{z_{it} t}\right)
    \prod_{k=1}^{K_t}p\left(\theta_{kt}\right).
  \end{align}
  Each term in the data likelihood is a Gaussian distribution with mean
  $\theta_{z_{it} t}$ and covariance $\sigma I$:
  \begin{align}
    \begin{aligned}
    p\left(y_{it} | \theta_{z_{it} t}\right) &= (2 \pi \sigma)^{-d/2}
    \exp{\left({-\frac{|| y_{it} - \theta_{z_{it}t} ||^2}{2 \sigma}}\right)}\\
    \therefore  \lim_{\sigma \to 0}-2\sigma\log p\left(y_{it} | \theta_{z_{it}
  t}\right) &= \|y_{it}-\theta_{z_{it}t}\|^2.
    \end{aligned}
  \end{align}
  Each term in the parameter prior corresponding to an old cluster is a Gaussian
  with mean $\theta_{p}$ and covariance  $\sigma_{p} I$ (after
  integrating out the old cluster parameter): 
  \begin{align}
  \begin{aligned}
    p\left(\theta_{kt}\right) &= (2 \pi \sigma_{p})^{-d/2}
    \exp{\left({-\frac{|| \theta_{kt} - \theta_{p} ||^2}{2
      \sigma_{p}}}\right)},
  \end{aligned}
  \end{align}
  where
  \begin{align}
    \begin{aligned}
    \theta_{p} &= \left\{\begin{array}{ll}
      \theta_{k(t-\dtk)} & \dtk > 0\\
                      \phi & \dtk = 0
                  \end{array}\right.\\
   \sigma_{p} &= \left\{\begin{array}{ll}
     \xi \dtk + \sigma_{k(t-\dtk)} & \dtk > 0\\
                    \rho & \dtk = 0
                \end{array}\right. .
    \end{aligned}
  \end{align}
  For new clusters, the parameters $\theta_{p}$ and
  $\sigma_{p}$ take into account the prior mean $\phi$ and
  covariance $\rho I$, and for revived clusters, they take into
  account the Gaussian transition with variance $\xi$ per time step, 
  along with the mean $\theta_{k(t-\dtk)}$ and covariance
  $\sigma_{k(t-\dtk)} I$ of the old parameter. As in the analysis of the
  Gibbs sampling algorithm, let $\xi = \tau \sigma$, and let
  $\sigma_{k(t-\dtk)} = \sigma/w_{k(t-\dtk)}$. Using these definitions,
  \begin{align}
  \begin{aligned}
    \therefore\lim_{\sigma\to0} -2\sigma\log p\left(\theta_{kt}\right) &=
    \left\{\begin{array}{ll}
      \gamma_{kt}\|\theta_{kt}-\theta_{k(t-\dtk)}\|^2
      & \dtk > 0\\
      0 & \dtk = 0
  \end{array}\right.\\
  \gamma_{kt} &= \left(\tau\dtk+w^{-1}_{k(t-\dtk)}\right)^{-1}.
  \end{aligned}
  \end{align}

  Finally, the assignment prior can be examined, using the fact that at each
  time step, the prior is marginally a Dirichlet process~\citep{Lin10_NIPS}.
  This allows the use of the CRP to expand the prior as follows:
  \begin{align}
    p\left(\{z_{it}\}_{i=1}^{N_t}\right) &=
    \left[\prod_{k : n_{kt}>0}\alpha_t^{\left[\dtk =
      0\right]}q_{kt}^{\left[\dtk >0\right]}\right]
    \left[\frac{1}{\alpha_t +
    \sum_{k=1}^{K_{t-1}}q_{kt}c_{kt}}\right]
    S\left(\alpha_t, \{q_{kt}, n_{kt}, c_{kt}\}_{k}\right),
  \end{align}
  where $S$ is a function determined by the CRP prior. 
  Again, following the analysis of the Gibbs sampling algorithm, let $\alpha_t =
  \frac{1-q^t}{1-q}\alpha_\nu$, $\alpha_\nu = \exp\left({-\frac{\lambda}{2\sigma}}\right)$,
  and $q_{kt} = q^\dtk = \exp\left({-\frac{Q\dtk}{2 \sigma}}\right)$. With 
  these definitions, $-2\sigma \log S \to 0$ as $\sigma \to 0$, and
  \begin{align}
    \therefore \lim_{\sigma\to0}-2\sigma\log
    p\left(\{z_{it}\}_{i=1}^{N_t}\right) &= -C+\sum_{k : n_{kt}>0}
      \left[\dtk=0\right]\lambda + Q\dtk,
  \end{align}
  where $C = \min\{\lambda, Q{\Delta t}_{1}, \dots, Q{\Delta t}_{K_{t-1}}\}$  
  does not depend on the cluster assignments or parameters.
  Combining the above results, the small-variance MAP estimation problem is
  equivalent to
  \begin{align}
  \begin{aligned}
    \lim_{\sigma\to0}&\min_{K_t, \{z_{it}\}_{i=1}^{N_t}, \{\theta_{kt}\}_{k=1}^{K_t}}-2\sigma\log\left(p\left(\{y_{it}\}_{i=1}^{N_t}, \{z_{it}\}_{i=1}^{N_t},
    \{\theta_{kt}\}_{k=1}^{K_t}\right)\right)\\
    = &\min_{K_t, \{z_{it}\}_{i=1}^{N_t}, \{\theta_{kt}\}_{k=1}^{K_t}} J_t - C.
  \end{aligned}
  \end{align}
  Thus, the small-variance MAP estimate is equal the global optimum clustering
  using the D-Means cost.
\end{proofof}



==> sdmeansbdmproof-arxiv.tex <==
\section{Proof of Modeling Capability of SD-Means}\label{app:sdmeansbdmproof}
\begin{proofof}{Theorem \ref{thm:sdmmodels}}
  \paragraph{Cluster Birth}
  Define 
  \begin{align}
    \delta \tilde{G}\equiv \left[\begin{array}{cc}
        0 & \krnmat{Y}{\Phi}\Gamma^{\frac{1}{2}}\\
      \Gamma^{\frac{T}{2}}\left(\krnmat{Y}{\Phi}\right)^T & 0 \end{array}\right].
  \end{align} 
  Therefore,
  \begin{align}
    G &= \tilde{G}+ \delta \tilde{G} , \quad \text{with }\tilde{G} = \left[\begin{array}{cc}
        \krnmat{Y}{Y} & 0 \\
        0 & \Gamma^{\frac{T}{2}}\krnmat{\Phi}{\Phi}\Gamma^{\frac{1}{2}} + \Omega
    \end{array}\right].
  \end{align}
By well-known matrix perturbation results for eigenvalues and
eigenvectors~\citep{Bauer60_NM,Davis69_AMS}, the eigenvalues of $G$ approach 
those of $\krnmat{Y}{Y}$ union those of
$\Gamma^{\frac{T}{2}}\krnmat{\Phi}{\Phi}\Gamma^{\frac{1}{2}}+\Omega$, while the
eigenvectors approach those of $\krnmat{Y}{Y}$ padded with zeros below,
and those of $\Gamma^{\frac{T}{2}}\krnmat{\Phi}{\Phi}\Gamma^{\frac{1}{2}}+\Omega$
padded with zeros above. Therefore, the spectral clustering produced by $G$ approaches
that of $\krnmat{Y}{Y}$, with diminishing influence from old clusters.
\paragraph{Cluster Death}
If a simple transformation is made to the eigenvalue equation for $G$,
  \begin{align}
    \begin{aligned}
      Gv &= \sigma v\\
      \frac{1}{Q\dtk} Gv &= \frac{\sigma}{Q\dtk} v\\
      G' v' &= \sigma' v',
    \end{aligned}
  \end{align}
  then 
  \begin{align}
    G' = \tilde{G}'+\delta\tilde{G}', \begin{aligned}
  \tilde{G'} &= \left[\begin{array}{cc}
                  0 & 0\\
                0 & e_k e_k^T\end{array}\right]\\
       \delta\tilde{G'} &= \frac{1}{Q\dtk}\left[\begin{array}{cc}
           \krnmat{Y}{Y} & \krnmat{Y}{\Phi}\Gamma^{\frac{1}{2}}\\
           \Gamma^{\frac{T}{2}}\left(\krnmat{Y}{\Phi}\right)^T &
           \Gamma^{\frac{T}{2}}\krnmat{\Phi}{\Phi}\Gamma^{\frac{1}{2}} + (I - e_k e_k^T) \Omega
          \end{array}\right],
    \end{aligned}
  \end{align}
  and the limiting argument holds once again
  because $\dtk \to \infty$ causes $\delta\tilde{G'} \to 0$. Therefore,
  there exists a eigenvector $v$ of $G$ such that $\lim_{\dtk\to\infty} v = e_{N_t+k}$.
  However, since $G$ is real and symmetric, its eigenvectors are
  orthonormal. Therefore, all other eigenvectors of $G$ satisfy
  $\lim_{\dtk\to\infty} v^Te_{N_t+k} = 0$; cluster $k$ has no influence
  on the components of the other eigenvectors.

  %The remaining step is to show that the columns of $V^\star$ satisfy the same
  %limits (despite the premultiplication by $\hat{\Gamma}^{-\frac{1}{2}}$). 
  %First, the eigenvector $v$ that approaches $e_{N_t+k}$ instead approaches
  %$e_{N_t+k}\gamma_{kt}^{-\frac{1}{2}}\propto e_{N_t+k}$. For other
  %eigenvectors $v$, by examination of the eigenvalue equation, 
  %the $(N_t+k)^{\text{th}}$ component satisfies
  %$|v_{N_t+k}| \propto \dtk^{-\frac{3}{2}}$ as $\dtk \to \infty$. Therefore,
  %$\gamma_{kt}^{-\frac{1}{2}}v_{N_t+k} \propto \dtk^{-1}$ as $\dtk \to \infty$.
  %Thus $\lim_{\dtk\to\infty} e^T_{N_t+k}\gamma_{kt}^{-\frac{1}{2}}v = 0$ and the result holds.
  \paragraph{Cluster Motion}
Suppose cluster death is ignored ($\Omega = 0$), and suppose $G$
has a single old cluster $k$ for notational simplicity -- the result generalizes
to the case of an arbitrary number of old clusters. Then $G$ is
\begin{align}
    G &=  \left[\begin{array}{cc}
        \krnmat{Y}{Y} & \krnmat{Y}{\Phi}\sqrt{\gamma_{kt}}\\
        \sqrt{\gamma_{kt}}\left(\krnmat{Y}{\Phi}\right)^T &
        \gamma_{kt} \krnmat{\Phi}{\Phi}
          \end{array}\right].
\end{align}
As $\dtk \to \infty$, $\gamma_{kt} \to 0$, so using the limiting proof from
earlier, the eigenvectors approach those of $\krnmat{Y}{Y}$ padded
with a 0 entry. There is also an eigenvector that approaches $e_{N_t+1}$, but
its eigenvalue approaches $0$, so it does not influence $V^\star$. Therefore,
the set of temporary clusters $l=1, \dots, \left|\clusa_t\right|$ approaches
that of spectral clustering with no old cluster information.
\end{proofof}

As a final note regarding cluster death and motion, if $Q > 0$
then the objective in (\ref{eq:clustermatching}) for old cluster $k$ with large
$\dtk$ is $\simeq \sum_{l=1}^{\left|\clusa_t\right|} c_{lk}Q\dtk$. If
$Q = 0$ on the other hand, the objective is $\simeq
\sum_{l=1}^{\left|\clusa_t\right|} c_{lk}(-\lambda)$. Since $Q, \lambda \geq 0$,
in the former case,
all clusters with large $\dtk$ are left uninstantiated (death), and in the latter,
all clusters with large $\dtk$ are reinstantiated (motion).
However, in either case, the data partitioning is unaffected by the old clusters.


%\begin{lemma}[Bauer-Fike 1960]\label{lem:bauerfike}
%  Let $A, \delta A\in\mathbb{R}^{n\times n}$, and let $A$ be symmetric.
%  Then for every eigenvalue
%  $\sigma'$ of $A+\delta A$, $\exists$ an eigenvalue $\sigma$ of $A$
%  such that
%  \begin{align}
%    |\sigma - \sigma'| \leq \|\delta A\|_2.
%  \end{align}
%\end{lemma}
%\begin{proof}
%  This result is proven in~\citep{Bauer60_NM}. 
%\end{proof}
%\begin{lemma}[Davis-Kahan 1969]\label{lem:daviskahan}
%  Suppose $A, \delta A\in \mathbb{R}^{n\times n}$ are symmetric operators.
%  Let $E\in\mathbb{R}^{n\times n}$, 
%  $E = \left[E_0 \, \, E_1\right]$ where $E_0 \in \mathbb{R}^{n\times k}$
%  is an orthonormal basis for a subspace spanned by
%  eigenvectors of $A$, and $E_1$ is an orthonormal basis
%  for the orthogonal space. $F_0$, $F_1$ are similarly
%  defined for $B=A+\delta A$.  Finally, define the matrices
%  $A_0, A_1, B_0, B_1$ via
%  \begin{align}
%    A = E\left(\begin{array}{cc}
%                  A_0 & 0\\
%                  0 & A_1\end{array}\right)E^T, \quad
%    B = F\left(\begin{array}{cc}
%                  B_0 & 0\\
%                  0 & B_1\end{array}\right)F^T.
%  \end{align}
%  If the spectrum of $A_0$ lies in an interval, and the spectrum of
%  $B_1$ lies distant from that interval by $\eta > 0$, then
%  $\eta \|E^T_1F_0\|_2 \leq \|\delta A\|_2$.
%\end{lemma}
%\begin{proof}
%  This result is proven in~\citep{Davis69_AMS}.
%\end{proof}
%\begin{proofof}{Theorem \ref{thm:sdmmodels}}
%  \paragraph{Cluster Birth}
%  Define 
%  \begin{align}
%    \delta \tilde{G}\equiv \left[\begin{array}{cc}
%        0 & Y^T\Phi\Gamma^{\frac{1}{2}}\\
%      \Gamma^{\frac{T}{2}}\left(Y^T\Phi\right)^T & 0 \end{array}\right].
%  \end{align} 
%  Therefore,
%  \begin{align}
%    G &= \tilde{G}+ \delta \tilde{G} , \quad \text{with }\tilde{G} = \left[\begin{array}{cc}
%        Y^TY & 0 \\
%        0 & \Gamma^{\frac{T}{2}}\Phi^T\Phi\Gamma^{\frac{1}{2}} + \Omega
%    \end{array}\right].
%  \end{align}
%By Lemma \ref{lem:bauerfike}, for every eigenvalue $\tilde{\sigma}$ of
%$\tilde{G}$ (and therefore for every eigenvalue $\tilde{\sigma}$ of $Y^TY$), there exists an eigenvalue $\sigma$ of $G$ such that
%\begin{align}
%  |\sigma - \tilde{\sigma}| \leq \|\delta\tilde{G}\|_2 \equiv \delta.
%\end{align}
%Let $\eta$ be the minimum distance between pairs of eigenvalues, and
%pick the elements of $\delta\tilde{G}$ small enough such that $\delta < \eta/4$. 
%Consider an eigenvalue $\tilde{\sigma}$ of $Y^TY$;
%let $\tilde{v}$ be its eigenvector (in $\tilde{G}$), and let $\tilde{V}_\perp$
%be the matrix of other eigenvectors of $\tilde{G}$. 
%Similarly, let $v$ be the eigenvector for the eigenvalue $\sigma$ of $G$ within $\eta/4$ of $\tilde{\sigma}$, 
%and $V_\perp$ be the matrix of other eigenvectors of $G$.
%By Lemma \ref{lem:daviskahan}, since $\tilde{\sigma}$ is separated from
%all other eigenvalues of $G$ by at least $\eta/2$,
%\begin{align}
%  \begin{aligned}
%  \frac{\eta}{2}\|\tilde{V}_\perp^Tv\|_2 &< \delta\\
%  \|\tilde{V}_\perp^Tv\|^2_2 &< \frac{4\delta^2}{\eta^2}\\
%  1-(\tilde{v}^Tv)^2 &< \frac{4\delta^2}{\eta^2}\\
%    \tilde{v}^Tv >& \sqrt{1-\frac{4\delta^2}{\eta^2}}\\
%    \|v-\tilde{v}\|_2 &<
%    \sqrt{2\left(1-\sqrt{1-\frac{4\delta^2}{\eta^2}}\right)}.
%  \end{aligned}
%\end{align}
%The third line is a result of $\tilde{G}$ being real and symmetric, and thus having
%an orthonormal basis of real eigenvectors. The fourth line follows since sign
%choice for eigenvectors is arbitrary. Therefore, by picking the elements of
%$\delta\tilde{G}$ small enough, one can set $\delta$ small enough to make 
%both $|\sigma - \tilde{\sigma}|$ and $\|v-\tilde{v}\|_2$ less than any $\epsilon
%> 0$. 
%
%Since $\tilde{G}$ is block diagonal with $Y^TY$ on the upper left block, 
%$V^\star \to \left[\begin{array}{cc} V^\star_{YY} & 0 \\
%  0 & \ast \end{array}\right]$. This is because the eigenvalues $\sigma$ determine which 
%eigenvectors $v$ appear as the column $\hat{\Gamma}^{-\frac{1}{2}} v$ in
%$V^\star$, and the eigenvalues $\sigma$ approach $\sigma_{YY}$. Further,
% premultiplying $v$ by $\hat{\Gamma}^{-\frac{1}{2}}$ does
%not affect the result, since the upper left block of $\hat{\Gamma}$ is $I$,
%and the lower right block of $\hat{\Gamma}$ is a constant as $Y^T\Phi\to 0$.
%
%\paragraph{Cluster Death}
%  If a simple transformation is made to the eigenvalue equation for $G$,
%  \begin{align}
%    \begin{aligned}
%      Gv &= \sigma v\\
%      \frac{1}{Q\dtk} Gv &= \frac{\sigma}{Q\dtk} v\\
%      G' v' &= \sigma' v',
%    \end{aligned}
%  \end{align}
%  then it is possible to reuse the limit proof for cluster birth, where
%  \begin{align}
%    \begin{aligned}
%  \tilde{G'} &= \left[\begin{array}{cc}
%                  0 & 0\\
%                0 & e_k e_k^T\end{array}\right]\\
%       \delta\tilde{G'} &= \frac{1}{Q\dtk}\left[\begin{array}{cc}
%           Y^TY & Y^T\Phi\Gamma^{\frac{1}{2}}\\
%           \Gamma^{\frac{T}{2}}Y^T\Phi^T &
%              \Gamma^{\frac{T}{2}}\Phi^T\Phi\Gamma^{\frac{1}{2}} + (I - e_k e_k^T) \Omega
%          \end{array}\right],
%    \end{aligned}
%  \end{align}
%  because $\dtk \to \infty$ causes $\delta\tilde{G'} \to 0$. Therefore,
%  there exists a eigenvector $v$ of $G$ such that $\lim_{\dtk\to\infty} v = e_{N_t+k}$.
%  However, since $G$ is real and symmetric, its eigenvectors are
%  orthonormal. Therefore, all other eigenvectors of $G$ satisfy
%  $\lim_{\dtk\to\infty} v^Te_{N_t+k} = 0$. 
%
%  The remaining step is to show that the columns of $V^\star$ satisfy the same
%  limits (despite the scaling by $\hat{\Gamma}^{-\frac{1}{2}}$). 
%  First, the eigenvector $v$ that approaches $e_{N_t+k}$ instead approaches
%  $e_{N_t+k}\gamma_{kt}^{-\frac{1}{2}}\propto e_{N_t+k}$. For other
%  eigenvectors $v$, by examination of the eigenvalue equation, 
%  the $(N_t+k)^{\text{th}}$ component satisfies
%  $|v_{N_t+k}| \propto \dtk^{-\frac{3}{2}}$ as $\dtk \to \infty$. Therefore,
%  $\gamma_{kt}^{-\frac{1}{2}}v_{N_t+k} \propto \dtk^{-1}$ as $\dtk \to \infty$.
%  Thus $\lim_{\dtk\to\infty} e^T_{N_t+k}v = 0$ and the result holds.
%
%\paragraph{Cluster Motion}
%If cluster death is ignored, and $G$ has a single old cluster $k$, $G$ becomes
%\begin{align}
%    G &=  \left[\begin{array}{cc}
%        Y^TY & Y^T\Phi\sqrt{\gamma_{kt}}\\
%        \sqrt{\gamma_{kt}}Y^T\Phi^T &
%          \gamma_{kt} \Phi^T\Phi
%          \end{array}\right]
%\end{align}
%as $\dtk \to \infty$, $\gamma_{kt} \to 0$, so using the limiting proof from
%earlier, the eigenvectors approach those of $Y^TY$ padded
%with a 0 entry. There is also an eigenvector that approaches $e_{N_t+1}$, but
%its eigenvalue approaches $0$, so it does not influence $V^\star$.
%
%The final step is to show that the bottom row of $V^\star$ doesn't approach 0. 
%For eigenvectors with nonzero $\sigma$, by examination of the eigenvalue
%equation, the $(N_t+k)^{\text{th}}$ component
%satisfies $|v_{N_t+k}| \propto \dtk^{-\frac{1}{2}}$ as $\dtk \to \infty$.
%Therefore, $\lim_{\dtk\to\infty} \gamma_{kt}^{-\frac{1}{2}} v_{N_t+k} \propto Y^T\Phi^Tv_{YY}$ 
%where $v_{YY}$ is an eigenvector of $Y^TY$. Since $Y^TY$ is symmetric, its
%eigenvectors are orthonormal, so the column $Y^T\Phi$ can not be orthogonal to all
%of its eigenvectors; hence, there exists a column in $V^\star$ such that
%the last entry approaches a nonzero constant. The result follows.
%\end{proofof}



==> sdmeansmonoproof-arxiv.tex <==
\section{Proof of Monotonicity in the SD-Means Infeasibility Cost}\label{app:sdmeansmonoproof}
\begin{lemma} [Ghouila-Houri 1962]\label{lem:totuni} Consider a matrix $A$ with $n$ rows of the form
  $r \in \mathbb{R}^{1\times n}$. 
  $A$ is totally unimodular
  iff for every subset $R$ of the rows, there is a partition of $R$,
  $R_+\cup R_- = R$, $R_+ \cap R_- = \emptyset$, such that
  \begin{align}
    \left[ \sum_{r \in R_+} r\right] - \left[\sum_{r \in R_-}r\right] \in
    \{0, 1, -1\}^{1\times n}.
  \end{align}
\end{lemma}
\begin{proof}
  This result is proven in~\citep{Schrijver03}. 
\end{proof}
\begin{proofof}{Lemma \ref{lem:totallyunimodular}}
The constraints of the linear program (\ref{eq:XCUpdate})
are as follows:
\begin{align}
  \begin{aligned}
        &\sum_{i=1}^{K_{t-1}} x_{ij} \leq 1 \,\, \forall\,\,
         j=1, \dots, A_t \\
         &\sum_{j=1}^{A_t} x_{ij} \leq 1\,\, \forall\,\, i=1, \dots, K_{t-1}\\
         &x_{ij} \geq 0\,\, \forall\,\, i=1, \dots, K_{t-1}, \, j=1,
         \dots, A_{t}.
  \end{aligned}
\end{align}
This set of linear constraints can be rewritten in the standard form 
of $Ax \leq b$. To show that $A$ is a totally unimodular
constraint matrix, we use Lemma \ref{lem:totuni}. Given any subset $R$ of
the rows of $A$, let $R'_+$ consist of the rows in $R$ corresponding
to the row constraints $\sum_{j=1}^{A_t} x_{ij} \leq 1$, and
let $R'_-$ consist of the rows in $R$ corresponding to the 
column constraints $\sum_{i=1}^{K_{t-1}} x_{ij} \leq 1$. Then since
every variable $x_{ij}$ in $X_C$ has a $1$ coefficient in exactly one row constraint
and a $1$ coefficient in exactly one column constraint, 
\begin{align}
    \left[ \sum_{r \in R'_+} r\right] - \left[\sum_{r \in R'_-}r\right] \equiv
    \tilde{r} \in \{0, 1, -1\}^{1\times N}.
\end{align}
Then, let $R''_+$ consist of the rows in $R$ corresponding to the individual
nonnegativity constraints $x_{ij} \geq 0$ in which $\tilde{r}$ has a 
$-1$ or $0$ entry in the column for $x_{ij}$, and let $R''_-$ be the remaining
nonnegativity constraint rows. Finally, let $R_+ = R'_+\cup R''_+$, and let
$R_- = R'_-\cup R''_-$. With this setting of $R_+/R_-$, the condition 
in Lemma \ref{lem:totuni} holds, and therefore $A$ is totally unimodular.
\end{proofof}
\begin{proofof}{Theorem \ref{thm:sdmeansmono}} We provide a proof
  that the steps (\ref{eq:XDUpdate}-\ref{eq:UUpdate}) are an alternating 
  minimization procedure for the optimization (\ref{eq:constrainedopt}).
  Thus, this proof is completed in two steps: the $U$ step (with $X$ fixed), and
  the $X$ step (with $U$ fixed).
  If both steps monotonically reduce the objective in
  (\ref{eq:constrainedopt}), then the result follows.

  For the $U$ step, the optimization
  (\ref{eq:constrainedopt}) with $X$ fixed is equivalent to the following:
  \begin{align}
  \begin{aligned}
    U^\star &= \argmin_{U} \|X - \overline{V^\star} U\|^2_F\\
  \text{s.t. } & U^TU = I, \quad U \in \mathbb{R}^{K\times K}.
\end{aligned}
  \end{align}
  This is a well-known optimization problem~\citep{Yu03_ICCV} that
  is solved by taking the singular value decomposition of $X^TRZ^\star$,
  and setting $U$ via
  \begin{align}
    \begin{aligned}
      X^T\overline{V^\star} &\overset{\text{svd}}{=} R\Sigma W^T\\
    U &\gets WR^T.
  \end{aligned}
  \end{align}
  which is precisely equation (\ref{eq:UUpdate}) in the SD-Means iteration. Thus,
  with a fixed $X$, equation (\ref{eq:UUpdate}) does not increase the objective
  in the optimization (\ref{eq:constrainedopt}).

  For the $X$ step, the optimization (\ref{eq:constrainedopt}) with fixed $U$ is
  equivalent to the following:
   \begin{align}
      \begin{aligned}
        X\gets \argmin_{\{x_{ij}\}}&
        \sum_{i=1}^{N_t+K_{t-1}}\sum_{j=1}^{A_t} x_{ij}\|e_j -
        \zeta^T_i\|^2 + \sum_{i=N_t+1}^{N_t+K_{t-1}} s_i \|\zeta_i\|^2\\
        \text{s.t. } &\sum_{j=1}^{A_t} x_{ij} = 1 \quad \forall i=1, \dots, N_t\\
        &s_i + \sum_{j=1}^{A_t} x_{ij} = 1 \quad \forall i=N_t+1, \dots,
        N_t+K_{t-1} \\
        &\sum_{i=N_t+1}^{N_t+K_{t-1}} x_{ij} \leq 1 \quad \forall
           j=1, \dots, A_t\\
           &x_{ij} \in \{0, 1\}, s_i \geq 0,
        \end{aligned}
  \end{align}
  where $s_i$ are slack variables for the old cluster rows $i=N_t+1, \dots,
  N_t+K_{t-1}$, since those rows may be set to 0.
  Noting that both the constraints and the objective are decoupled between the $X_D$
  and $X_C$ blocks, this optimization can be split into two separate optimizations. 
  
  The first sets the rows of $X_D$, where each row is set individually, as they
  are decoupled from the others in the optimization. Since the rows of $\overline{V^\star}U$ are
  normalized, the magnitudes of all elements in $\zeta_i$ are less than $1$.
  Thus, minimizing $\sum_{j=1}^{A_t}x_{ij}\|e_j-\zeta^T_i\|^2$ involves
  selecting the entry $j^\star$ with the maximum value in $\zeta_i$, and setting
  $x_{ij^\star} = 1$, $x_{ij} = 0 \, \, \forall j \neq j^\star$. This is
  precisely equation (\ref{eq:XDUpdate}) in the SD-Means iteration.
  
  The second decoupled component of the optimization sets $X_C$. The rows of
  $X_C$ are, however, not decoupled, and so must be set simultaneously. The
  resulting optimization to solve is (with row indices $i$ shifted down by
  $N_t$)
  \begin{align}
      \begin{aligned}
        X_C\gets \argmin_{\{x_{ij}\}}&
        \sum_{i=1}^{K_{t-1}}\sum_{j=1}^{A_t} x_{ij}\|e_j -
        \zeta^T_i\|^2 + \sum_{i=1}^{K_{t-1}} s_i \|\zeta_i\|^2\\
        \text{s.t. } & s_i + \sum_{j=1}^{A_t} x_{ij} = 1 \quad \forall i=1,
        \dots, K_{t-1}\\
        &\sum_{i=1}^{K_{t-1}} x_{ij} \leq 1 \quad \forall
           j=1, \dots, A_t\\
           &x_{ij} \in \{0, 1\}, s_i \geq 0.
        \end{aligned}
  \end{align}
  Substituting $s_i = 1-\sum_{j}^{A_t} x_{ij}$ into the constraints and
  objective yields
  \begin{align}
      \begin{aligned}
        X_C\gets \argmin_{\{x_{ij}\}}&
        \sum_{i=1}^{K_{t-1}}\|\zeta_i\|^2 + \sum_{j=1}^{A_t} x_{ij}\left(\|e_j -
        \zeta^T_i\|^2 - \|\zeta_i\|^2\right)\\
        \text{s.t. } & \sum_{j=1}^{A_t} x_{ij} \leq 1 \quad \forall i=1,
        \dots, K_{t-1}\\
        &\sum_{i=1}^{K_{t-1}} x_{ij} \leq 1 \quad \forall
           j=1, \dots, A_t\\
           &x_{ij} \in \{0, 1\}.
         \end{aligned}\label{eq:XCintegeropt}
  \end{align}
  Removing the constants $\|\zeta_i\|^2$ from the objective, and
  reformulating the term $\|e_j - \zeta^T_i\|^2 - \|\zeta_i\|^2 =
  e^T_je_j - 2e^T_j\zeta_i = 1-2\zeta^T_ie_j$ yields
  an optimization that is equivalent to equation (\ref{eq:XCUpdate}) in the
  SD-Means iteration, except for the integer
  constraints. However, by Lemma \ref{lem:totallyunimodular}, the optimization
  (\ref{eq:XCUpdate}) has a totally unimodular constraint matrix, and as such it
  produces an integer solution. Since (\ref{eq:XCUpdate}) is a relaxation of
  (\ref{eq:XCintegeropt}), and produces a feasible solution to (\ref{eq:XCintegeropt}), solving
  (\ref{eq:XCUpdate}) is equivalent to solving (\ref{eq:XCintegeropt}). Thus,
  with fixed $U$, equations (\ref{eq:XDUpdate}-\ref{eq:XCUpdate}) do not
  increase the objective in the optimization (\ref{eq:constrainedopt}).
\end{proofof}


==> simpleblock-arxiv.tex <==
\begin{tikzpicture}[scale=.75, every node/.style={transform shape}]
  %triangle
  \Vertex[x=1, y=1, L=$y_{1}$]{y1}
  \Vertex[x=-1, y=2, L=$y_{2}$]{y2}
  \Vertex[x=0, y=0, L=$y_{3}$]{y3}
  \tikzstyle{LabelStyle}=[above right]
  \Edge[label=$1$](y1)(y2)
  \tikzstyle{LabelStyle}=[above right]
  \Edge[label=$1$](y2)(y3)
  \tikzstyle{LabelStyle}=[below right]
  \Edge[label=$1$](y3)(y1)
  %old cluster node
  \tikzset{VertexStyle/.style = {fill = gray, shape=circle, minimum size=17pt,
  line width=1pt, draw}}
  \Vertex[x=-3, y=1, L=$\theta'_1$]{c1}
  \tikzstyle{LabelStyle}=[above left=0.06]
  \Edge[label=$\beta$](c1)(y1)
  \tikzstyle{LabelStyle}=[above left]
  \Edge[label=$\beta$](c1)(y2)
  \tikzstyle{LabelStyle}=[below left]
  \Edge[label=$\beta$](c1)(y3)
\end{tikzpicture}







==> spectralrelaxation-arxiv.tex <==
\section{Spectral Relaxation of the Small-Variance MAP Filtering
Problem}\label{sec:spectralrelaxation}

Iterative clustering methods are inherently local; they
do not necessarily find a globally optimal clustering
and are susceptible to getting trapped in a poor local 
cost minimum. One way of addressing this locality is 
through \emph{spectral relaxation} of the clustering 
problem~\citep{Zha01_NIPS,Kulis12_ICML}, where some
of the clustering constraints are removed, yielding
a relaxed problem that may be solved globally via 
eigendecomposition. The relaxed solution may then be
refined to produce a feasible clustering that is typically
less susceptible to local clustering minima. 
The following sections will discuss such a spectral 
clustering algorithm, developed from the small-variance MAP
filtering problem for the Markov DDP Gaussian mixture.


%One way to enhance the applicability and flexibility of D-Means is to create a
%spectral relaxation of the cluster cost minimization problem~\citep{Zha01_NIPS,Kulis12_ICML}, 
%and use it to develop a spectral clustering algorithm. In contrast to iterative clustering
%algorithms like D-Means, only a notion of pairwise similarity between datapoints
%is required to use spectral clustering, and it is known to be capable of capturing clusters of arbitrary
%shape~\citep{Ng02_NIPS}. Spectral clustering has been used in wide variety of applications, 
%such as segmentation of images~\citep{Shi00_IEEETPAMI}, grading of breast cancer
%histopathology~\citep{Doyle08_ISBI}, clustering data with arbitrary structure~\citep{Ng02_NIPS},
%speech separation~\citep{Bach06_JMLR}, topological mapping~\citep{Valgren07_ICRA}, and blog relationship
%discovery~\citep{Chi07_KDD}. 
%Thus, the goal of the following sections is to
%provide a spectral clustering algorithm developed from the small-variance MAP
%filtering problem for the Markov DDP Gaussian mixture.

%\subsection{Matrix Definitions of $y_{it}$, $\theta_{kt}$, $\phi_{kt}$}\label{subsec:specmatdefs}
%The first step towards creating a spectral relaxation of the optimization of the cost (\ref{eq:DMeansObj}) 
%is to reformulate it as a matrix trace optimization. Define the matrix of data
%vectors, $Y$; the matrix of old parameters, $\Phi$; an indicator column for
%index $i$, $e_i$ (dimension will be clear from context); 
%and an indicator column for all observations in cluster $k$, $f_k$, as follows: 
%\begin{align}
%\begin{aligned}
%  Y &= \left[\begin{array}{cccc}y_{1t}& y_{2t}& \cdots& y_{N_t
%    t}\end{array}\right]\in\mathbb{R}^{d\times N_t}\\
%  \Phi &= \left[\begin{array}{cccc}\phi_{1t} &
%      \phi_{2t}  & \cdots & \phi_{K_{t-1}t}  
%  \end{array}\right] \in\mathbb{R}^{d\times K_{t-1}}\\
%  f_k &= \sum_{i\in\indices_{kt}} e_i \in \mathbb{R}^{N_t}.
%\end{aligned}
%\end{align}
%Given these definitions, the following identities hold for the datapoints
%$y_{it}$, old cluster parameters $\phi_{kt}$, and current cluster
%parameters $\theta_{kt}$:
%\begin{align}
%\begin{aligned}
%  y_{it} &= Ye_i\\
%  \phi_{kt} &= \Phi e_k\\
%  \theta_{kt} &= \frac{\gamma_{kt}}{\gamma_{kt}+n_{kt}}\Phi e_k +
%  \frac{1}{\gamma_{kt}+n_{kt}}Yf_k,
%\end{aligned} 
%\end{align}
%where the equation for $\theta_{kt}$ follows from the parameter update
%(\ref{eq:paramupdate}).
%\subsection{Distance Terms} The prior-weighted sum of squares component of the objective
%(\ref{eq:DMeansObj}) can be rewritten as the sum of matrix traces,
%\begin{align}
%  \begin{aligned}
%    J^{\text{dist}}_t &\equiv \sum_{k\in\clusa_t} \gamma_{kt}\|\theta_{kt}-
%    \phi_{kt}\|^2 
%    +\sum_{i\in\indices_{kt}} \|y_{it} -\theta_{kt}\|^2\\
%   &=\tr{Y^TY} + \tr{\Gamma^{\frac{T}{2}} \Phi^T\Phi\Gamma^{\frac{1}{2}}} -
%  \tr{F_1^TY^TYF_1}- \tr{F_0^TY^TYF_0}\\
%    &\qquad - \tr{E_0^T\Gamma^{\frac{T}{2}}
%  \mathrm{diag}(\Phi^T\Phi)\Gamma^{\frac{1}{2}}E_0}
%  - 2\tr{ E_0^T\Gamma^{\frac{T}{2}}\Phi^TYF_0},
%\end{aligned}\label{eq:specdistcost}
%\end{align}
%where $\mathrm{diag}(\Phi^T\Phi)$ is a diagonal matrix with the diagonal
%elements of $\Phi^T\Phi$, the matrices $F_0$, $F_1$, and $E_0$ are defined as
%\begin{align}
%  \begin{aligned}\label{eq:EFdefs}
%F_0^T &= \left[\begin{array}{c}
%     \frac{f^T_1}{\sqrt{\gamma_{1t}+n_{1t}}} \\
%        \vdots\\
%        \frac{f^T_{K_{t-1}}}{\sqrt{\gamma_{{K_{t-1}}t}+n_{{K_{t-1}}t}}}
%    \end{array}\right] \, \, 
%  F_1^T = \left[\begin{array}{c}
%      \frac{f^T_{(K_{t-1}+1)}}{\sqrt{n_{(K_{t-1}+1)t}}} \\
%        \vdots\\
%        \frac{f^T_K}{\sqrt{n_{K_tt}}}
%        \end{array}\right]\\
%%\Gamma = \left[\begin{array}{ccc}
%%              \gamma_1 & &\\
%%              & \hspace{-.3cm}\ddots &\\
%%            & & \hspace{-.3cm}\gamma_{K_{t-1}}\end{array}\right]\\
% E_0^T &=  \left[\begin{array}{ccc}
%     \frac{\sqrt{\gamma_{1t}}}{\sqrt{\gamma_{1t}+n_{1t}}}& &0\\
%              & \ddots &\\
%            0& &
%          \frac{\sqrt{\gamma_{{K_{t-1}}t}}}{\sqrt{\gamma_{{K_{t-1}}t}+n_{{K_{t-1}}t}}}\end{array}\right],
%  \end{aligned}
%\end{align}
%and $\Gamma\in\mathbb{R}^{{K_{t-1}}\times {K_{t-1}}}$ is a square diagonal matrix with the
%$\gamma_{kt}$ along the diagonal for each old cluster $k \in \{1, \dots,K_{t-1}\}$.
%\subsection{Penalty Terms}
%The sum of the penalty terms in (\ref{eq:DMeansObj}),
%\begin{align}
%  J^{\text{pen}}_t &\equiv \sum_{k\in\clusa_t} \lambda\ind{\dtk} + Q\dtk, \label{eq:jpen}
%\end{align}
%can be broken into the new and old cluster penalties. The sum of the new cluster costs 
%in (\ref{eq:jpen}) is straightforward to put in a matrix trace formulation:
%\begin{align}
%  \sum_{k\in\clusa_t} \lambda\ind{\dtk} &=
%  \sum_{k\in\clusa_t} \frac{f^T_{k}f_k}{n_{kt}}
%  \lambda =\tr{ F_1^T \lambda I F_1}.\label{eq:jpen1}
%\end{align}
%However, the $Q\dtk$ revival costs in (\ref{eq:jpen}) for the old clusters are not as simple to include,
%due to the non-constant terms on the diagonal. Thus, the penalty is modified as follows:
%\begin{align}
%  \sum_{k\in\clusa_t} Q\dtk \simeq \sum_{k\in\clusa_t}
%  \frac{n_{kt}}{\gamma_{kt}+n_{kt}}Q\dtk.
%\end{align}
%This modification preserves the value of the original penalty 
%when $n_{kt} = 0$ (the cluster is uninstantiated) or when $\dtk = 0$ (the cluster is
%new), as it incurs a penalty of $0$ in these cases. 
%Otherwise, if
%$\gamma_{kt}$ is large, the cluster was very popular in past timesteps;
%therefore, instantiating the cluster has a low cost. Likewise, if
%$\gamma_{kt}$ is small, the cluster was not popular, and
%$\frac{n_{kt}}{\gamma_{kt}+n_{kt}} \approx 1$, so it is more costly to instantiate
%it. Thus, the modified penalty makes sense in that ``the rich get richer'',
%similar to the behavior of the Dirichlet process.  Expressed in matrix trace notation, 
%\begin{align}
%  \sum_{k\in\clusa_t} \frac{n_{kt}}{\gamma_{kt}+n_{kt}}Q\dtk 
%  &= \sum_{k\in\clusa_t} \frac{f^T_{k} f_k}{\gamma_{kt} + n_{kt}} Q\dtk 
%  =\tr{ \Omega F^T_0  F_0},
%\end{align}
%where $\Omega\in\mathbb{R}^{{K_{t-1}}\times {K_{t-1}}}$ is a diagonal matrix with the $Q\dtk$
%along the diagonal.
%Unfortunately, $\tr{\Omega F_0^TF_0} \neq \tr{F^T_0 \Omega F_0}$,
%because the diagonal elements of $\Omega$ are not constant. However, $F^T_0F_0
%= I - E^T_0E_0$; and since $E_0$ is diagonal, $\Omega$
%commutes with $E_0$. Thus,
%\begin{align}
%  \sum_{k\in\clusa_t} \frac{n_{kt}}{\gamma_{kt}+n_{kt}}Q\dtk = \tr{\Omega
%  - E^T_0 \Omega E_0}, \label{eq:jpen2}
%\end{align}
%and the final formulation of the cluster penalties in equation 
%(\ref{eq:jpen}) is the sum of the results from equations (\ref{eq:jpen1}) and
%(\ref{eq:jpen2}),
%\begin{align}
%  J^{\text{pen}}_t &\simeq \hat{J}^{\text{pen}}_t =  \tr{\Omega - E^T_0 \Omega E_0} + \tr{ F_1^T \lambda
%  I F_1}.
%\end{align}
%

\subsection{Spectral Relaxation}
In order to perform a spectral relaxation of the KD-Means clustering
problem (\ref{eq:krnmin}), the standard technique is to first express it
as a constrained matrix trace minimization~\citep{Zha01_NIPS,Kulis12_ICML}. 
However, it is not possible to include the old cluster penalties
$\sum_{k\in\clusa_t}Q\dtk$ in such a formulation. Thus, the penalty 
is modified as follows:
\begin{align}
  \sum_{k\in\clusa_t} Q\dtk \simeq \sum_{k\in\clusa_t}
  \frac{n_{kt}}{\gamma_{kt}+n_{kt}}Q\dtk.
\end{align}
This modification preserves the value of the original penalty 
when $n_{kt} = 0$ (the cluster is uninstantiated) or when $\dtk = 0$ (the cluster is
new), as it incurs a penalty of $0$ in these cases. 
Otherwise, if $\gamma_{kt}$ is large, the cluster was very popular in past timesteps;
therefore, instantiating the cluster has a low cost. Likewise, if
$\gamma_{kt}$ is small, the cluster was not popular, and
$\frac{n_{kt}}{\gamma_{kt}+n_{kt}} \approx 1$, so it is more costly to instantiate
it. Thus, the modified penalty makes sense in that ``the rich get richer'',
similar to the behavior of the Dirichlet process. Further, this modification
strictly reduces the cost of any clustering, and thus preserves the lower
bounding property of the exact spectral relaxation.

Given this modification, it is possible to rewrite the kernelized clustering
problem (\ref{eq:krnmin}) as a trace minimization,
\begin{align}
  \begin{aligned}
    \min_{Z} \tr{\krnmat{Y}{Y}} +
    \tr{\Gamma^{\frac{T}{2}} \krnmat{\Phi}{\Phi}\Gamma^{\frac{1}{2}}} + \tr{\Omega -
    \lambda I}-\tr{Z^T\hat{\Gamma}^{\frac{T}{2}}(G-\lambda
    I)\hat{\Gamma}^{\frac{1}{2}}Z}, 
  \end{aligned}\label{eq:spectralmin}
\end{align}
where $Z$, $G$ and $\hat{\Gamma}$ are defined as
\begin{align}
 % \begin{aligned}
\label{eq:ZGdefine}
\hspace{-.3cm}Z = \left[\begin{array}{ccc}
    c_1 & \dots & c_{K_t} 
\end{array}\right] \Xi ,
\,  \,
\hat{\Gamma} = \left[\begin{array}{cc}
    I & 0 \\
    0 & \Gamma
\end{array}\right] , \, \,
G =\hat{\Gamma}^{\frac{T}{2}}\left[\begin{array}{cc}
    \krnmat{Y}{Y}& \krnmat{Y}{\Phi}\\
    \left(\krnmat{Y}{\Phi}\right)^T& 
  \mathrm{diag}(\krnmat{\Phi}{\Phi}) + \Gamma^{-1}\Omega
  \end{array}\right]\hat{\Gamma}^{\frac{1}{2}}.
%\end{aligned}
\end{align}
In the above, $c_k\in\{0, 1\}^{N_t+K_{t-1}}$ is an indicator vector
for cluster $k$ ($c_{ki} = 1, \, i \leq N_t$ indicates that datapoint $i$
is assigned to cluster $k$, and $c_{kk'} = 1, \, k' > N_t$ 
indicates that cluster $k$ is linked to old cluster $k'$, where at most one component
$c_{kk'}, \, k'> N_t$ can be set to 1),
the matrix $\Gamma\in\mathbb{R}^{{K_{t-1}}\times {K_{t-1}}}$ is a square diagonal matrix with the
$\gamma_{kt}$ along the diagonal for each old cluster $k \in \{1,
\dots,K_{t-1}\}$, and $\Xi\in\mathbb{R}^{K_t\times K_t}$ is a square matrix with
the value $\left(\gamma_{kt}+n_{kt}\right)^{-\frac{1}{2}}$ along the diagonal
for each cluster $k\in \{1, \dots, K_t\}$.

If the problem is relaxed by removing all constraints on $Z$
except for $Z^T\hat{\Gamma}Z = I$, (\ref{eq:spectralmin})
is equivalent to solving
\begin{align}
  &\begin{aligned}\label{eq:relaxedopt}
    Z^\star = &\argmax_{Z} \tr{Z^T\hat{\Gamma}^{\frac{T}{2}}(G-\lambda
    I)\hat{\Gamma}^{\frac{1}{2}}Z}\\
    &\quad \mathrm{s.t. }\, \, Z^T\hat{\Gamma}Z = I,
  \end{aligned}
\end{align}
for which the set of global optimum solutions is~\citep{Yu03_ICCV}
\begin{align}
  Z^\star &\in \left\{V^\star U : U\in\mathbb{R}^{\left|\clusa_t\right|\times \left|\clusa_t\right|}, \, U^T = U^{-1}\right\}\\
  V^\star &=\hat{\Gamma}^{-\frac{1}{2}}\left[v_1, \dots, v_{\left|\clusa_t\right|}\right]\in
  \mathbb{R}^{(N_t+{K_{t-1}})\times {\left|\clusa_t\right|}}, \label{eq:UVdefine}
\end{align}
where $\{v_1, \dots, v_{\left|\clusa_t\right|}\}$ are unit eigenvectors of $G$ whose corresponding eigenvalues
are greater than $\lambda$.
Note that $\left|\clusa_t\right| \neq K_t$ in general; $K_t$ accounts for clusters
that were created in a previous time step but are not active in the current time
step. Therefore, $\left|\clusa_t\right| \leq K_t$, where equality occurs when all old clusters $k$
satisfy $n_{kt} > 0$.

%Due to the relaxation of some of the constraints on $Z$ in the optimization,
%$V^\star$ does not directly provide a feasible clustering of the data. However, 
%equation (\ref{eq:spectralmin}) evaluated at $V^\star$ does provide a lower bound on the global
%optimum of the D-Means cost (\ref{eq:DMeansObj}), since the
%modification to the original old cluster revival penalty is a lower bound on the 
%original, and since $V^\star$ is found by solving a relaxed version of the 
%clustering problem.

\subsection{Finding a Feasible Solution}\label{subsec:specfeasible}
Given the set of global minimum solutions of the relaxed problem $\{V^\star U :
  U^T = U^{-1}\}$, the next step is
to find an indicator matrix $X$ that yields the label assignments and old/new
cluster correspondences, and a unitary matrix $U$, such that $X$ as close as possible to $V^\star U$ in some sense.
Previous work on spectral clustering obtained a feasible clustering $X$ 
by minimizing the Frobenius norm between $X$ and row-normalized
$V^\star U$~\citep{Yu03_ICCV},
\begin{align}
  X^\star, U^\star &= \argmin_{X, U} \|X -
  \text{diag}^{-\frac{1}{2}}(V^\star V^{\star T})V^\star U\|^2_F.
\end{align}
However, there are a number of issues with this procedure related to the last
${K_{t-1}}$ rows of $V^\star$. The first is that some of the last ${K_{t-1}}$ rows may be comprised entirely of
$0$ elements, making the row normalization operation undefined. This occurs
because only a subset of the eigenvectors of $G$ are used; if an old cluster
is uninstantiated in the current dataset, its eigenvector may not appear in
the columns of $V^\star$, resulting in a row of $0$ elements for that old cluster.
In practice, a row of $0$ elements in $V^\star$ can possibly appear as a row of
small numbers, because $V^\star$ is the solution of a relaxed problem and
is not guaranteed to contain the structure outlined by (\ref{eq:ZGdefine}). 
This makes it difficult to tell whether a row 
in $V^\star$ should not be normalized because it corresponds to a row of $0$
elements, or it should be normalized because it corresponds to an old cluster with a very small
$\gamma_{kt}$ or large $n_{kt}$. The second issue is that the columns of $V^\star$ may
be permuted arbitrarily, so it is impossible to know a priori which columns
correspond to new clusters, and which of the remaining columns correspond to 
which old cluster.
The last issue related to finding $X$ is that the last ${K_{t-1}}$ rows of $X$
\emph{exclude} each other from selecting the same $1$ element
in order to preserve a 1-1 correspondence between old and new clusters. Thus,
past greedy discrete optimization methods~\citep{Yu03_ICCV} cannot be used in
this context without modification.

In the following, the subscripts $D$ and $C$ refer to the first $N_t$ and last $K_{t-1}$ 
rows of a matrix, respectively (i.e.~$D$ corresponds to the current batch of
data, $C$ corresponds to old clusters). 
To find a clustering from $V^\star$, we first normalize each of its 
rows in $V^\star_D$; and for every row corresponding
to old cluster $k$ in $V^\star_C$, normalize the row if its squared
norm is greater than $\frac{0.5}{\gamma_{kt}+N_t}$, and otherwise set it to 0. The
resulting row-normalized matrix $\overline{V^\star}$
captures the notion that the old cluster rows should only be normalized
if they are large enough, in the sense that they have a magnitude closer to
$\frac{1}{\sqrt{\gamma_{kt} + {N_t}}}$ than to $0$.
Given $\overline{V^\star}$, we propose the nonlinear integer optimization
(\ref{eq:constrainedopt}) to find a feasible clustering of the data: 
\begin{align}
  \begin{aligned}\label{eq:constrainedopt}
    X^\star, U^\star &= \argmin_{X, U} \|X - \overline{V^\star} U\|^2_F\\
  \text{s.t. } & X_D \bm{1} = \bm{1}\\
        & X_C \bm{1} \leq \bm{1}\\
        & X_C^T \bm{1} \leq \bm{1}\\
        & X \in \{0, 1\}^{(N_t+K_{t-1})\times A_t}\\
        & U^TU = I \quad  U \in \mathbb{R}^{A_t\times A_t},
 \end{aligned}
\end{align}
where $\bm{1}$ is a column consisting of all $1$ entries (dimension is clear from context). The optimization
(\ref{eq:constrainedopt}) minimizes the Frobenius between a cluster
assignment matrix $X$ and the normalized global relaxed solution $\overline{V^\star}U$.
The first constraint on $X$ enforces that each datapoint is assigned to a single cluster,
the next two enforce the one-to-one correspondence between old and current clusters,
and the third enforces that $X$ is an indicator matrix. Finally, $U$ is constrained
to be unitary, so that $V^\star U$ is within the set of global optima of (\ref{eq:relaxedopt}).




==> temporalgraph-arxiv.tex <==
\begin{tikzpicture}[scale=0.75, every node/.style={transform shape}]
  %First block, Bottom triangle
  \Vertex[x=0, y=1, L=$y_{1}$]{y1}
  \Vertex[x=1, y=1.5, L=$y_{2}$]{y2}
  \Vertex[x=1, y=0.5, L=$y_{3}$]{y3}
  \Edge(y1)(y2)
  \Edge(y2)(y3)
  \Edge(y3)(y1)
  %First block, top triangle
  \Vertex[x=0, y=3, L=$y_{4}$]{y4}
  \Vertex[x=1, y=3.5, L=$y_{5}$]{y5}
  \Vertex[x=1, y=2.5, L=$y_{6}$]{y6}
  \Vertex[x=2, y=3, L=$y_{7}$]{y7}
  \Edge(y4)(y5)
  \Edge(y4)(y6)
  \Edge(y4)(y7)
  \Edge(y5)(y6)
  \Edge(y5)(y7)
  \Edge(y6)(y7)
  %cross edge or two
  \Edge(y1)(y6)
  \Edge(y2)(y4)
    %Second block top triangle
  \Vertex[x=5, y=3.5, L=$y_{1}$]{y9}
  \Vertex[x=5.5, y=2.5, L=$y_{2}$]{y10}
  \Edge(y9)(y10)
  %Second block bottom line seg
  \Vertex[x=4.5, y=0.5, L=$y_{3}$]{y11}
  \Vertex[x=5.5, y=1.5, L=$y_{4}$]{y12}
  \Edge(y11)(y12)
  %old cluster nodes
  \tikzset{VertexStyle/.style = {fill = gray, shape=circle, minimum size=17pt,
  line width=1pt, draw}}
  \Vertex[x=4, y=3, L=$\theta'_1$]{c1}
  \Vertex[x=3.5, y=1, L=$\theta'_2$]{c2}
  \Vertex[x=7.5, y=3, L=$\theta'_1$]{c3}
  \Vertex[x=7.5, y=1, L=$\theta'_2$]{c4}
  \Edge(c1)(y9)
  \Edge(c1)(y10)
  \Edge(c2)(y11)
  \Edge(c2)(y12)
  \Edge(c2)(y10)
  %summary rectangles/lines
  \node[color=gray, dashed, line width=.5pt, draw, fill=none, fit=(y1)(y2)(y3)] (rect2) {};
  \node[color=gray, dashed, line width=.5pt, draw, fill=none, fit=(y4)(y5)(y6)(y7)] (rect1) {};
  \node[color=gray, dashed, line width=.5pt, draw, fill=none, fit=(y9)(y10)(c1)] (rect3) {};
  \node[color=gray, dashed, line width=.5pt, draw, fill=none, fit=(y11)(y12)(c2)] (rect4) {};
  \node[draw=none, fill=none, above=.2 of rect1] (t) { {\large $t$}};
  \node[draw=none, fill=none, right=3 of t] (t1) { {\large $t+1$}};
  \node[draw=none, fill=none, right=1.7 of t1] (t2) { {\large $t+2$}};
  \draw[->, bend left=30, gray, line width=.5pt, dashed] (rect1.east) to (c1);
  \draw[->, bend right=30, gray, line width=.5pt, dashed] (rect2.east) to (c2);
  \draw[->, bend left=30, gray, line width=.5pt, dashed] (rect3.east) to (c3);
  \draw[->, bend right=30, gray, line width=.5pt, dashed] (rect4.east) to (c4);
  \node[draw=none, fill=none, right=.3 of c3] (dots3) { {\huge$\cdots$}};
  \node[draw=none, fill=none, right=.3 of c4] (dots4) { {\huge$\cdots$}};
\end{tikzpicture}







==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}
